Time Series Synthesis Using the Matrix Profile for Anonymization

Publishing and sharing data is crucial for the data mining community, allowing collaboration and driving open innovation. However, many researchers cannot release their data due to privacy regulations or fear of leaking confidential business information. To alleviate such issues, we propose the Time Series Synthesis Using the Matrix Profile (TSSUMP) method, where synthesized time series can be released in lieu of the original data. The TSSUMP method synthesizes time series by preserving similarity join information (i.e., Matrix Profile) while reducing the correlation between the synthesized and the original time series. As a result, neither the values for the individual time steps nor the local patterns (or shapes) from the original data can be recovered, yet the resulting data can be used for downstream tasks that data analysts are interested in. We concentrate on similarity joins because they are one of the most widely applied time series data mining routines across different data mining tasks. We test our method on a case study of ECG and gender masking prediction. In this case study, the gender information is not only removed from the synthesized time series, but the synthesized time series also preserves enough information from the original time series. As a result, unmodified data mining tools can obtain near-identical performance on the synthesized time series as on the original time series.

==> insert/alg_tsaump.tex <==
\begin{algorithm}[ht]
  \caption{TSSUMP Algorithm}\label{alg:tssump}
  \begin{algorithmic}[1]
  \footnotesize
    \Procedure{TSSUMP}{$T, m, n_\text{batch}, n_\text{iter}$}
      \State $n \gets \textsc{GetLength}(T)$ 
      \State $MP^{TT}_m,MPI^{TT}_m \gets \textsc{MatrixProfile}(T,m)$
      \State $\hat{T} \gets $ sample $n$ values from $\mathcal{N}(0,1)$
      \For{$0$ \textbf{to} $n_\text{iter} - 1$}
        \State $I \gets \textsc{GetBatchIdx}([0,\cdots,n-m], n_\text{batch})$ %sample without replacement from 
        \State $J \gets \textsc{GetNeighborIdx}(MPI^{TT}_m,I)$
        \State $K \gets \textsc{GetNonNeighborIdx}([0,\cdots,n-m],I,J)$
        \State $\mathcal{L}_{\text{local}} \gets  \textsc{GetLocalLoss}(T_{I,m},\hat{T}_{I,m})$ \Comment{Eq. \ref{eq:pri_loss}.}
        \State $\mathcal{L}_{\text{dist}} \gets  \textsc{GetDistLoss}(MP^{TT}_m[I],\hat{T}_{I,m},\hat{T}_{J,m})$ \Comment{Eq. \ref{eq:dist_loss}.}
        \State $\mathcal{L}_{\text{identity}} \gets  \textsc{GetIdentityLoss}(\hat{T}_{I,m},\hat{T}_{J,m},\hat{T}_{K,m})$ \Comment{Eq. \ref{eq:id_loss}.}
        \State $\mathcal{L} \gets \mathcal{L}_{\text{local}} + \mathcal{L}_{\text{dist}} + \mathcal{L}_{\text{identity}}$
        \State $\hat{T} \gets \hat{T} + \textsc{GetGradientUpdate}(\mathcal{L})$
        \State $\hat{T} \gets $z$\textsc{Normalization}(\hat{T})$
      \EndFor
      \State \Return $\hat{T}$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> insert/fig_Trace_CLU.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{insert/figure/fig_tsne_2.pdf}
    \caption{Samples from the Trace dataset of the UCR Archive are visualized with $t$-SNE~\cite{TSNE} algorithm. 
    Datapoint colors correspond to class labels.
    \textit{Top)} Points are annotated with an index to show their positions are relatively conserved. 
    \textit{Bottom)} Colored blocks are used to demonstrate these groups of points' relative positioning to one another.}
    \label{fig:visaulization}
\end{figure}

==> insert/fig_complex.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{insert/figure/fig_complex_1.pdf}
    \caption{
    Higher complex time series has a higher complexity score after the ``stretch".
    }
    \label{fig:complex}
\end{figure}

==> insert/fig_distpro.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{insert/figure/fig_distpro_0.pdf}
    \caption{The distance profile~$DP^{AB}_{i,m}$ shows the nearest neighbor (the most similar subsequence) of the query $T^A_{i,m}$ in $T^B$.}
    \label{fig:distpro}
\end{figure}

==> insert/fig_dm.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{insert/figure/fig_dm_0.pdf}
    \caption{The original time series~$T$ (green), its TSAUMP-anonymized proxy~$\hat{T}$ (red), and their matrix profiles.
    The discovered discords are colored in yellow.}
    \label{fig:dm}
\end{figure}


==> insert/fig_matpro_aa.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{insert/figure/fig_matpro_aa_0.pdf}
    \caption{The Matrix Profile~$MP^{AA}_m$ highlights the repeated patterns in $T^A$.}
    \label{fig:matpro_aa} 
\end{figure}

==> insert/fig_matpro_ab.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{insert/figure/fig_matpro_ab_0.pdf}
    \caption{The Matrix Profile~$MP^{AB}_m$ reveals the unique patterns that only occur in $T^A$ but not $T^B$.}
    \label{fig:matpro_ab}
\end{figure}

==> insert/fig_mm.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{insert/figure/fig_mm_0.pdf}
    \caption{The original time series~$T$ (green), its TSAUMP-anonymized proxy~$\hat{T}$ (red), and their matrix profiles.
    The discovered motifs are colored in yellow.}
    \label{fig:mm}
\end{figure}


==> insert/fig_mmdm_toy.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{insert/figure/fig_mmdm_toy_1.pdf}
    \caption{The original time series~$T$ (green), its TSAUMP-anonymized proxy~$\hat{T}$ (red), and their matrix profiles. 
    \textit{Top)} The motif mining problem. 
    \textit{Bottom)} The discord mining problem.}
    \label{fig:mmdmtoyfig}
\end{figure}


==> insert/fig_segment.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{insert/figure/fig_segment_0.pdf}
    \caption{The original time series~$T$ (green), its TSAUMP-anonymized proxy~$\hat{T}$ (red), and their corrected arc crossing (CAC) curve returned by the FLUSS algorithm.
    The location of the minimal value in the CAC reveals the regime change.
    The CACs of both $T$ and $\hat{T}$ are almost identical.}
    \label{fig:segment}
\end{figure}


==> insert/fig_toy_discord.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics{insert/figure/fig_toy_discord_0.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> insert/fig_tsaump.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{insert/figure/fig_tsaump_1.pdf}
    \caption{
    The anonymization function~$f(\cdot)$ generates the anonymized time series~$\hat{T}$ from the input time series~$T$.
    The original $T$ cannot be recovered from $\hat{T}$, and $s(d(T)) \approx s(d(\hat{T}))$.
    }
    \label{fig:tsaump}
\end{figure}


==> insert/tab_ad_results.tex <==
% \footnotesize
\begin{table}[ht]
    \centering
    \caption{AD scores on 12 models. Lower Prediction Difference scores is one indicator of TSAUMP's success at synthesizing a proxy for real data.}
    \label{tab:ad_results}
    \begin{tabular}{cc||cc|c}
        \multicolumn{2}{c||}{\textbf{Method}} & Real & Synth. & Pearson Corr. \\
        \hline
        \hline
        \multirow{2}{*}{LOF~\cite{breunig2000lof}} & AD Acc. & 22.40 & 20.96 & {\multirow{2}{*}{ 0.4950}}\\
        & Pred. Diff. & \multicolumn{2}{c|}{0.208} & \\
        \hline
        \multirow{2}{*}{IForest~  \cite{liu2008iForest}} & AD Acc. & 13.04 & 15.04 & {\multirow{2}{*}{0.1432}}\\
        & Pred. Diff. & \multicolumn{2}{c|}{0.1272} & \\
        \hline
        \multirow{2}{*}{OCSVM} & AD Acc. & & & \\
        & Pred. Diff. & & & \\
        \hline
        \multirow{2}{*}{Autoreg} & AD Acc. & & & \\
        & Pred. Diff. & & & \\
        \hline
        \multirow{2}{*}{AE~\cite{kramer1991nonlinear}} & AD Acc. & 17.10 & 14.17 & {\multirow{2}{*}{0.45310}}\\
        & Pred. Diff. & \multicolumn{2}{c|}{0.1211} & \\
        \hline % recheck AE numbers when they're done running
        \multirow{2}{*}{VAE~\cite{kingma2013auto}} & AD Acc. & & & \\
        & Pred. Diff. & & & \\
        \hline
        \multirow{2}{*}{DeepSVDD~\cite{pmlr-v80-ruff18a}} & AD Acc. & & & \\
        & Pred. Diff. & & & \\
        \hline
        \multirow{2}{*}{AnoGAN~\cite{schlegl2017unsupervised}} & AD Acc. & & & \\
        & Pred. Diff. & & & \\
        \hline
        \multirow{2}{*}{LSTM~\cite{hochreiter1997long}} & AD Acc. & & & \\
        & Pred. Diff. & & & \\
        \hline
        \multirow{2}{*}{GRU~\cite{cho2014properties}} & AD Acc. & & & \\
        & Pred. Diff. & & & \\
        \hline
        \multirow{2}{*}{DAGMM~\cite{zong2018dagmm}} & AD Acc. &  & & {\multirow{2}{*}{0.}}\\
        & Pred. Diff. & \multicolumn{2}{c|}{0.} & \\
        \hline
        \multirow{2}{*}{MP~\cite{yeh2016matrix}} & AD Acc. & 34.00 & 24.44 & {\multirow{2}{*}{0.6039}}\\ 
        & Pred. Diff. & \multicolumn{2}{c|}{0.2416} & \\
        \hline
    \end{tabular}
\end{table}

==> insert/tab_segment.tex <==
\begin{table}[ht]
    \centering
    \caption{Comparison of different semantic segmentation methods on original and synthesized time series.}
    % \resizebox{0.99\columnwidth}{!}{
    \footnotesize
    \label{tab:segment}
    \begin{tabular}{l||cc}
     & Original & Synthesized \\ \hline \hline
    FLUSS & 1.47 & 1.50 \\
    Binseg & 3.61 & 3.81 \\
    BottomUp & 3.05 & 2.84 \\
    KernelCPD & 3.56 & 3.50 \\
    Window & 3.31 & 3.34 \\
    \end{tabular}
% }
\end{table}



==> insert/tab_toys.tex <==
\begin{table}[ht]
    \centering
    \caption{The results of the top-1 motif and top-1 discord comparisons of the Matrix Profile on \texttt{T} and \texttt{TSAUMP(T)} on a toy experiment and random noise stress test. Reported scores are averaged over 100 runs.}
    \label{tab:toy_results}
    \begin{tabular}{c|c|c}
         & Top-1 Motif & Top-1 Discord \\ \hline
        \textbf{Toy} & 0.0117 & 0.0243 \\
    \end{tabular}
\end{table}
